Learning to Predict Gradients for Semi-Supervised Continual Learning

A key challenge for machine intelligence is to learn new visual concepts without forgetting the previously acquired knowledge. Continual learning is aimed towards addressing this challenge. However, there is a gap between existing supervised continual learning and human-like intelligence, where human is able to learn from both labeled and unlabeled data. How unlabeled data affects learning and catastrophic forgetting in the continual learning process remains unknown. To explore these issues, we formulate a new semi-supervised continual learning method, which can be generically applied to existing continual learning models. Specifically, a novel gradient learner learns from labeled data to predict gradients on unlabeled data. Hence, the unlabeled data could fit into the supervised continual learning method. Different from conventional semi-supervised settings, we do not hypothesize that the underlying classes, which are associated to the unlabeled data, are known to the learning process. In other words, the unlabeled data could be very distinct from the labeled data. We evaluate the proposed method on mainstream continual learning, adversarial continual learning, and semi-supervised learning tasks. The proposed method achieves state-of-the-art performance on classification accuracy and backward transfer in the continual learning setting while achieving desired performance on classification accuracy in the semi-supervised learning setting. This implies that the unlabeled images can enhance the generalizability of continual learning models on the predictive ability on unseen data and significantly alleviate catastrophic forgetting. The code is available at \url{https://github.com/luoyan407/grad_prediction.git}.

==> depd/fig_anal_confusion_noise_u.tex <==
\begin{figure*}[!t]
	\centering
	\begin{minipage}[t]{0.40\textwidth}
        \centering
        \vspace{0pt}
        \includegraphics[width=1\linewidth]{fig/analysis/gem_noise_u_confusion}
        \caption*{ResNet GEM $\mathcal{U}(-1,1)$}
    \end{minipage} \hfill
    \begin{minipage}[t]{0.40\textwidth}
        \centering
        \vspace{0pt}
        \includegraphics[width=1\linewidth]{fig/analysis/gem_gp_noise_u_confusion}
        \caption*{ResNet GEM $\mathcal{U}(-1,1)$ + proposed}
    \end{minipage}
	\caption{\label{fig:confusion_u}
    	Confusion matrix using random noise as predicted gradients. The noise follows a uniform distribution $\mathcal{U}(-1,1)$.
    % 	that is evaluated at every training stage for all the tasks by substituting the noise for the predicted gradients.
	}
\end{figure*}

==> depd/fig_loss_vs_accuracy_effnet.tex <==
\begin{figure}[!t]
	\centering
	\begin{tabular}{cc}
	\footnotesize{~~~~~~~EffNet GEM} & \footnotesize{~~~~~~~EffNet DCL}  \\
	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/gem_effnet_loss_ledg}    } &
	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/dcl_effnet_loss}    } \vspace{-1ex} \\
	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/gem_effnet_accuracy}} &
	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/dcl_effnet_accuracy}} \vspace{-1ex} \\
	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/gem_effnet_fitloss} } &
	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/dcl_effnet_fitloss} } \\
	\end{tabular}
	\vspace{-2ex}
	\caption{\label{fig:loss_vs_accuracy_effnet}
    	Plots of improvement with the proposed method over training loss curves (top), validation accuracy curves (middle), and fitness loss curves (bottom) on iCIFAR-100. % with various pairs of methods.
    	}
\end{figure}
% \subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/gem_resnet_loss}    } \hfill
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/dcl_resnet_loss}    } \hfill
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/gem_effnet_loss}    } \hfill
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/dcl_effnet_loss}    } \\
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/gem_resnet_accuracy}} \hfill
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/dcl_resnet_accuracy}} \hfill
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/gem_effnet_accuracy}} \hfill
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/dcl_effnet_accuracy}} \\
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/gem_resnet_fitloss} } \hfill
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/dcl_resnet_fitloss} } \hfill
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/gem_effnet_fitloss} } \hfill
% 	\subfloat{\includegraphics[width=0.23\textwidth]{fig/analysis/dcl_effnet_fitloss} } \\

==> depd/tab_analysis_iCIFAR_sensitivity.tex <==
\begin{table}[!t]
	\centering
	\caption{\label{tbl:cifar_sensitivity}
	    \REVISION{Sensitivity of using hyperparameters across datasets. Specifically, we experiment with hyperparameters optimized on MNIST-R on iCIFAR-100. For each analysis, one of hyperpaprameters would be changed while retaining the other hyperpaprameters for clarity. Hyperpaprameter is abbreviated as HyperP below.}
	    }
		%we denote a setting as (\textit{training set}, \textit{test set}).
	\vspace{-2ex}
	\adjustbox{width=1.0\columnwidth}{
	\begin{tabular}{L{12ex} L{12ex} C{9ex} C{9ex} C{9ex}}
		\toprule
		Method & HyperP & Accuracy & BWT & FWT \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
		 PG (FT) & $p=0.15$ & 65.21 & 0.0164 & 0.0070  \\
		 PG (FT) & $\alpha=0.001$ & 68.12 & 0.0668 & 0.0019  \\
		 PG (FT) & $\lambda=0.30$ & 68.43 & 0.0601 & 0.0047  \\
		 \midrule
		 PG (COS) & $p=0.15$ & 66.50 & 0.0145 & -0.0023  \\
		 PG (COS) & $\alpha=0.001$ & 67.09 & 0.0639 & 0.0077  \\
		 PG (COS) & $\lambda=0.30$ & 66.77 & 0.0586 & 0.0141  \\ 
		\bottomrule	
	\end{tabular}}
% 	\vspace{-2ex}
\end{table}

==> depd/tab_hyperparameters_supv.tex <==
\begin{table}[t]
	\centering
	\caption{\label{tbl:hyper_supv}
		Hyperparameters w.r.t. the proposed method in the SSL setting. We follow \cite{Zhang_AISTATS_2021} for the hyperparameters that are not specific to the proposed method.
	}
 	\vspace{-2ex}
	\adjustbox{width=1.0\columnwidth}{
		\begin{tabular}{l c c c c}
			\toprule
			Dataset  & Backbone & $\alpha$ & $\lambda$ & $h_{\omega}$ \\ \midrule
			SVHN  & Conv-Large \cite{Tarvainen_NeurIPS_2017} & 0.001 & 2.00 & (128,32) \\
			CIFAR-10  & Conv-Large &  0.001 & 1.00 & (128,32) \\
			CIFAR-100  & Conv-Large &  0.001 & 1.00 & (128,32) \\
			\bottomrule
	\end{tabular}}
\end{table}

==> depd/tab_semi_diffsize.tex <==
\begin{table}[!t]
	\centering
	\caption{\label{tbl:semi_diffsize}
	    \REVISION{Effects of using different size of labeled data for semi-supervised classification on CIFAR-10 and CIFAR-100. For both datasets, the number of training images is 50K. The experimental protocol is identical to the one in \cite{Zhang_AISTATS_2021}. Rep. is short for reproduced.}
	    }
		%we denote a setting as (\textit{training set}, \textit{test set}).
	\vspace{-2ex}
	\adjustbox{width=1.0\columnwidth}{
	\begin{tabular}{L{18ex} C{4ex} C{4ex} C{4ex} C{4ex} C{4ex} C{4ex} }
		\toprule
		Dataset & \multicolumn{3}{c}{CIFAR-10} & \multicolumn{3}{c}{CIFAR-100} \\
		\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7}
% 		\#Images & 50K & 50K & 50K & 50K & 50K & 50K \\
		\#Labels & 1K & 2K & 4K & 6K & 8K & 10K \\
		\midrule
		FastSWA & 6.6 &   5.7 &   5.0 & - & - & 28.0 \\
		MG (ResNet-26 + shake-shake) & 6.3 &  5.2 &  4.1 & 26.7 &  25.1 &  22.9 \\
		\midrule
		 MG (Conv-Large) & 11.79 & 10.21 & 7.82 & 34.67 & 32.21 & 30.74  \\
% 		 PG (FT) &  &  &  & & & \\
		 PG (COS) & 10.34 & 9.24 & 7.58 & 34.35 &  31.71 & 30.37  \\
		\bottomrule	
	\end{tabular}}
% 	\vspace{-2ex}
\end{table}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> sec/sec_broader_impact.tex <==


\section*{Broader Impact}

This research studies a new learning paradigm that leverages information in the training steps to improve the descent. 
Being model agnostic and general, the method will advance and enrich the fundamental research in machine learning. The more efficient and effective search of local minimum that facilitates the learning process will also bring significant impacts in developing automatic systems in a wide range of domains including education, healthcare, e-commerce, and many more. As other machine learning methods, systems derived with the method may fall short in performance or interpretability. While the proposed method shows improved performance, depending on specific domains or applications with varied requirements, precautions may need to be taken accordingly before using the automatic systems. This work, targeting an generic learning framework rather than a specific task or application, does not foresee particular ethical concerns in any specific areas or societal consequences. For a broader impact, we release the software of our research to the public. The source code is %attached in the Supplementary Materials. It is also 
available at \url{https://rb.gy/qx1kuu}.


%This work studies a problem that leverages the information learned from samples to guide the learning process to hike down efficiently to the local minimum. 
%This work is generic and its ultimate motivation is to benefit a broad variety of areas, \eg healthcare, education, economy, and etc, for human's material well-being.
%On the other hand, as the proposed method facilitates the learning process for applications, rather than implementing specific applications, 
%we believe that even the proposed work is modified for malevolent purposes, the resulting method would not harm humans and other morally relevant beings. 
%Because the proposed method is an essential tool for applications and is neutral to applications, and any modified version of this work cannot determine or re-shape the downstream applications. 
% In summary, this work has no direct link to malevolent applications.
%Therefore, this work does not present any foreseeable societal consequence.

% reference: The Ethics of Artificial Intelligence (published paper) and my imagination

%---------------previous version starts from here------------------
% This work studies a problem that leverages the information learned from samples to guide the learning process to hike down efficiently to the local minimum. Our primary motivation is to provide a new perspective on the gradient descent that looks for a new direction to descend. The proposed method is generic and can apply to train models for other problems. As a result, the boosted model could used for both malicious and benevolent purposes. Nevertheless, the algorithmic impact of the proposed method has no direct link to malevolent applications and does not break the code of ethics.

% reference: https://hub.packtpub.com/machine-learning-ethics-what-you-need-to-know-and-what-you-can-do/

%---------------requirement starts from here------------------
% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}
